Composed Image Retrieval for Remote Sensing

This work introduces composed image retrieval to remote sensing. It allows to query a large image archive by image examples alternated by a textual description, enriching the descriptive power over unimodal queries, either visual or textual. Various attributes can be modified by the textual part, such as shape, color, or context. A novel method fusing image-to-image and text-to-image similarity is introduced. We demonstrate that a vision-language model possesses sufficient descriptive power and no further learning step or training data are necessary. We present a new evaluation benchmark focused on color, context, density, existence, quantity, and shape modifications. Our work not only sets the state-of-the-art for this task, but also serves as a foundational step in addressing a gap in the field of remote sensing image retrieval. Code at: https://github.com/billpsomas/rscir

==> tex/fig_presentation.tex <==
{
%\scriptsize
\footnotesize
\centering
\newcommand{\myg}[1]{\includegraphics[width=0.135\textwidth,valign=c]{#1}}

\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}ccc@{}}
   
    \mycaption{Query Image} & 
    \mycaption{Query Text} & 
    \mycaption{Retrieved Image} \\
    
    \myg{fig/examples/airplane159.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{purple}}} & 
    \myg{fig/examples/airplane073.jpg} \\
    \mc{3}{(a) Color}\\

    \mc{3}{\vspace{-2.1ex}}\\
    \myg{fig/examples/swimmingpool408.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{circular}}} & 
    \myg{fig/examples/swimmingpool314.jpg} \\

    \mc{3}{(b) Shape
    }\\

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/forest520.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{fine}}} & 
    \myg{fig/examples/forest081.jpg} \\

    \mc{3}{(d) Texture
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/christmastreefarm410.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{dense}}} & 
    \myg{fig/examples/christmastreefarm161.jpg} \\

    \mc{3}{(e) Density
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/airplane388.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{bigger}}} & 
    \myg{fig/examples/airplane697.jpg} \\

    \mc{3}{(c) Size
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/wastewaterplant614.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{four}}} & 
    \myg{fig/examples/wastewaterplant691.jpg} \\

    \mc{3}{(f) Quantity
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/denseresidential690.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{by the sea}}} & 
    \myg{fig/examples/coastalmansion573.jpg} \\

    \mc{3}{(g) Context
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/parkingspace002.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{with cars}}} & 
    \myg{fig/examples/parkinglot453.jpg} \\

    \mc{3}{(h) Addition
    }\\ 

\end{tabular}
}

==> tex/method_0.tex <==
\section{Method}
\label{sec:method}


\begin{figure*}[t]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},width=1.0\linewidth]{fig/cir_method.pdf}
\vspace{-8pt}
\caption{
\emph{\ours: A Weighted Composed Image Retrieval Method.} It utilizes a dual-encoder approach to process both \textcolor{imagequerycolor}{image $y$} and \textcolor{textquerycolor}{text $t$} queries. Initially, the \textcolor{imagequerycolor}{image query} is passed into a visual encoder $f$ and the \textcolor{textquerycolor}{text query} into a text encoder $g$, producing corresponding $d$-dimensional representations. Subsequently, it calculates similarity scores with the representations in the image dataset. These scores are then normalized and combined using a convex combination controlled by a $\lambda \in [0,1]$. Finally, an argmax operation identifies the most relevant and visually similar image, with attributes adjusted according to the text query, resulting in the \textcolor{retrievedimagecolor}{retrieved image $x$.}}
\label{fig:method}
\vspace{-14pt}
\end{figure*}


\subsection{Preliminaries}
\label{sec:prelim}

In composed image retrieval, the goal is to retrieve images based on an \emph{composed image-text query}, that is, a query that consists of a \emph{visual} part, the query image, and a \emph{textual} part, the query text. In this work, we introduce composed image retrieval into remote sensing. To do so, we focus on unisource retrieval, establishing a benchmark and an evaluation protocol.

\gkako{
Let's denote the query image as \(y\).  
Let \(C\) be the set of all possible classes and \(A_c^y\) represent the set of all attributes of the class \(c\) in \(y\). Then, we define:

\begin{equation}
\omega_{y} := \{A_c^y | c \in C \}
\end{equation}

The set \(A_c^y\) may include attributes such as color, shape, size, texture, density, context, quantity, or existence. If a class \(c\) is not present in image \(y\), then we define \(A_c^y = \emptyset\), indicating that the attribute set for class \(c\) in image \(y\) is empty.

Given a query text \(t \in \cT\), where $\cT$ is the text space, we define a function \(T: (\Omega \times \cT) \rightarrow \Omega\) that modifies the attribute sets based on the query text \(t\).

In the case that a previously empty set becomes non-empty after modification by \(T\), we refer to the task as \emph{class addition}. In any other case, we refer to it as \emph{attribute modification}. For example, as shown in~\autoref{fig:presentation}, consider an image \(y\) depicting a rectangular swimming pool. Given the query text \(t\) as ``circular,'' \(T\) acts on the \(A_c^y\) attribute set corresponding to the class ``swimming pool,'' changing the attribute from ``rectangular'' to ``circular''.

}

%\previous{
%In particular, let's denote the query image as $y$. 
%In this image, there can be multiple objects, each belonging to a different class. Suppose there are $N$ objects, each object $i$ belonging to a class $C_i$. We represent the set of all objects in the image $y$ along with their respective classes as a set of tuples: 
%If $C$ is the set of all possible classes and $A_k$ the set of all the attributes of the k-th object in $y$, we can map $y$ to a set of tuples:

%\begin{equation}
%\Omega(y) := \{(C_k, A_k) | k \in 1, 2, ..., K \}
%\end{equation}
%$A_k$ can include descriptions of color, shape, size, texture, density, context, quantity or existence. 

%A given query text $t$ acts on the set of tuple altering the attribute sets through a mapping function $T$:

%\begin{equation}
%T(\Omega(y)) = \{(C_k, A'_k) | k \in 1, 2, ..., K \}
%\end{equation}

%For example, as shown in~\autoref{fig:presentation}, an image $y$ of a rectangular swimming pool and the query text $t$ ``circular'' acts on the $A_k$ set of attributes that corresponds to the class ``swimming pool'' and it changes the attribute ``rectangular'' to ``circular''. Note that here we treat ``existence'' and ``non existence'' as attributes so a text query $t$ can introduce a new class. In that case we refer to the task as \emph{class addition}, in any other case we refer to the task as \emph{attribute modification}.
%}

The query image $y$ and the text query $t$ are jointly referred to as the \emph{composed query}, $q = (y, t)$. Given an image dataset $X$, the goal is to retrieve images from $X$ that are best described by the set $T(\Omega(y))$.

%${(O_1, C_1(y)), (O_2, C_2(y)), \ldots, (O_N, C_N(y))}$.

%\gkakoc{I think that we do not need the C to be a function of y, if we keep this notation I think C only is ok. Is this notation used in CV CIR?} 

%Here, $O_i$ represents the $i$-th object in the image and $C_i$ represents the class of the $i$-th object. In the case of single-class images, the formulation is simplified, as image $y$ depicts only one object of class $C$.

%We extend the formulation to incorporate additional attributes for each object in the image. Let $a_i$ denote the attribute of object $O_i$, which can be one of the following: color, shape, size, texture, density, or quantity. The query text $t$ can represent modifications related to $a_i$ for each object $O_i$ in the image. Additionally, $t$ may include instructions for the addition of one or more new objects, denoted as $O_k$, where $k$ is the index of the added object. Each $O_k$ is associated with its class $C_k$ and attributes $a_k$. We represent the enriched set of all objects of an image $y$ as a combination of the \nikos{following set of triplets:}

%original set of objects and their classes, along with their attributes, and any additional objects specified in the query text: \((O_1, C_1(y), a_1), \ldots, (O_N, C_N(y), a_N),\) \((O_{N+1}, C_{N+1}, a_{N+1}), \ldots, (O_{N+k}, C_{N+k}, a_{N+k})\) 

%\gkakoc{k here is the number of added objects while previously was an index, maybe to do it $K$}. 

%In this representation, the first $N$ tuples correspond to the objects originally present in the image $y$, while the tuples from $N+1$ to $K$ represent the additional objects introduced as per the query text $t$.

%\gkakoc{Although I like the story/ formulation, I am not sure if it fits what we do. I think that the formulation should be described after the actual/ final evaluation protocol. Nevertheless, maybe we should merge the (o, c) and the extended (o, c, a) formulation and keep the second, i.e. merge the second and third paragraphs and maybe avoid continuing the counting from N+1. We could only refer to an extra addition to exist in a set of tuples of the retrieved image. Maybe $\mathcal{Y}$ is the set of (o, c, a) attributes of the query image and $\mathcal{X}$ for the retrieved or maybe something else}

%Query image with query text are jointly referred to as the \emph{composed query}, $q=(y,t)$. Given an image dataset $X$, the goal is to retrieve images from $X$ whose classes have remained the same, but an attribute $a_i$ of an object $O_i$ has been modified, or one or more objects of new classes are being added. We refer to former as \emph{attribute modification} and to latter as \emph{class addition}. Retrieval amounts to ranking images $x \in X$ according to their \emph{composed similarity} $s(q, x) \in \real$ to the query $q$.

We rely on a pre-trained vision-language model that consists of a \emph{visual encoder} $f: \cI \to \real^d$ and a \emph{text encoder} $g: \cT \to \real^d$, which map respectively input images from image space $\cI$ and words\footnote{With the term \emph{words}, we shall refer to both words and sentences.} from text space $\cT$ to the same embedding space of dimension $d$. Using those encoders, we extract a visual embedding $\vy = f(y) \in \real^d$ and text embedding $\vt = g(t) \in \real^d$ for the query. Similarly, the embedding of an image $x \in X$ are denoted by $\vx = f(x) \in \real^d$. All embeddings are $\ell_2$-normalized. 

We also define a \emph{composed encoder} $h: \cI \times \cT \to \real^d$ in order to map the composed query $q$ to $\vq = h(q) = h(y, t) \in \real^d$

Unless explicitly specified otherwise, we employ the cosine similarity between the query and the database features as our chosen metric for measuring similarity.

%Given the visual-language model, the goal in this work is to represent the composed query in the same embedding space as images and text. That is, define a \emph{composed encoder} $h: \cI \times \cT \to \real^d$ such that the composed query $q$ is mapped to $\vq = h(q) = h(y, t) \in \real^d$, again $\ell_2$-normalized. For any image $x \in X$, this allows us to express the composed similarity as the cosine similarity
%\begin{equation}
%	s(q, x) \defn h(q)\tran f(x) = h(y, t)\tran f(x).
%\label{eq:sim}
%\end{equation}
%Thus, given the encoders $f, g$, the goal is to define $h$.

%This retrieval process involves two primary scenarios:
%\begin{enumerate}
%    \item \textbf{Attribute Modification:} In this scenario, the retrieved images will contain objects similar to those in the query image \( y \), but with modifications in their attributes as specified by the query text \( t \). The classes of the objects \( C_i(y) \) remain unchanged, but their attributes \( a_i \) differ in accordance with the modifications described in \( t \).
%    \item \textbf{Class Addition:} Here, the retrieved images will not only include objects present in the original query image \( y \) but also new objects as dictated by \( t \). These new objects, denoted as \( O_{N+k} \), belong to classes \( C_{N+k} \) that were not present in the original image \( y \) but are introduced through the query text. The challenge lies in identifying images that correspond to this expanded set of objects and classes.
%\end{enumerate}

%------------------------------------------------------------------------------

\subsection{Baselines}
\label{sec:base}
We compare our method to two baselines: The unimodal baseline, in which only one of the image/text queries is used and the linear baseline, in which we use a naive combination of the two.

\subsubsection{Unimodal}
Baselines based on unimodal queries depend solely on similarity using just one type of query method. We denote: \emph{text-only} by $h_T(y, t) := g(t)$ and \emph{image-only} by $h_V(y, t) := f(y)$. Unimodal baseline is expected to fail since the final similarity cannot embody information from both image and text sources.


\subsubsection{Sum}
A widely used baseline in the literature combines the two unimodal approaches by summation, $h_S(y, t):= g(t) + f(y)$. The drawback of this approach is that the distribution of the image-to-text similarities are quite different than the image-to-image similarities in the CLIP space. Specifically the features that come from same modalities have similarities significantly greater than the cross-modal similarities, making it an approach biased in favor of the image query.
\subsection{\ours}
\label{sec:base}

%The text and visual similarities after a normalization process, referred to as ``Text + Image (N)'' in~\autoref{}. A normal distribution is fit to the similarities between the text query $g(t)$ and all the database images $f(x)$ for $x \in X$, and similarly for the image query $f(y)$. For each distribution, the corresponding cumulative distribution function is used to transform the similarities. The two distributions of transformed similarities are closer to uniform. Finally, the similarities are combined by summation.
% Despite its simplicity, is shown to outperform some of the existing methods in the literature. \bp{Last sentence is not correctly located here - results}

In our proposed method, \ours, we estimate the similarities of the image query and the text query with the database. Then we perform similarity normalization in order to have a starting point of equal contribution from both modalities. Finally we use the weighted average of the two similarity sets using a modality control parameter $\lambda$:

\subsubsection{Similarity Normalization} 
In order to ensure that both image and text queries contribute equally to the retrieval we are normalizing their similarities with the database. We first transform the empirical distribution of similarity scores into a standard normal distribution. This is achieved by standardizing each similarity point using the mean and standard deviation of the sample set. Subsequently, we apply the cumulative distribution function (CDF) of the standard normal distribution to the standardized data, resulting in values that range between 0 and 1. Assuming the standardized data adhere to a normal distribution, this transformation yields data that approximates a uniform distribution. Transforming data into a uniform distribution diminishes the influence of outliers and reduces skewness, smoothing any excessively peaked distributions. This approach leads to more robust similarity scores.

\subsubsection{The modality control parameter $\lambda$}
After normalizing the similarities we can control the influence of each modality using a parameter $\lambda$ as a weight. Here $\lambda=0$ refers to image-only retrieval, $\lambda=1$ to text-only retrieval and $\lambda=0.5$ to equal contribution of the image and text queries. The full \ours method can be summarized in ~\autoref{fig:method}
%------------------------------------------------------------------------------


==> tex/teaser_old.tex <==
%------------------------------------------------------------------------------
% place teaser between title and abstract
\makeatletter
\apptocmd\@maketitle{{\teaser{}}}{}{}
\makeatother
%------------------------------------------------------------------------------
\newcommand{\myfig}[1]{\includegraphics[width=0.125\textwidth,valign=c]{#1}}
\newcommand{\mycaption}[1]{{\rotatebox[origin=c]{0}{\footnotesize#1}}}

\newcommand{\mytextquery}[1]{{\rotatebox[origin=c]{0}{\footnotesize#1}}}
\setlength{\tabcolsep}{5pt}
\newcommand{\boxcolor}{\setlength{\fboxrule}{.8pt} \color{textquerycolor}}
\newcommand{\boxcolorim}{\setlength{\fboxrule}{.8pt} \color{imagequerycolor}}

\newcommand{\teaser}{%
%------------------------------------------------------------------------------
\vspace{-15pt}
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}ccccccc@{}}


 {\boxcolorim \fbox{\myfig{fig/teaser/image_query_1.jpg}}} &
    \myfig{fig/teaser/image_1_retrieval_l10.jpg} &
    %\myfig{fig/teaser/image_query.jpg} &
    \myfig{fig/teaser/image_1_retrieval_l05.jpg} & 
    %\myfig{fig/teaser/image_query.jpg} &
    \myfig{fig/teaser/image_1_retrieval_l00.jpg} &
    {\boxcolor \fbox{\parbox[c][0.125\textwidth][c]{0.125\textwidth}{\centering \texttt{\textcolor{black}{with a roundabout}}}}} \\

    \addlinespace[2.5pt] 
    {\boxcolorim \fbox{\myfig{fig/teaser/image_query_2.jpg}}} &
    \myfig{fig/teaser/image_2_retrieval_l10.jpg} &
    %\myfig{fig/teaser/image_query.jpg} &
    \myfig{fig/teaser/image_2_retrieval_l05.jpg} & 
    %\myfig{fig/teaser/image_query.jpg} &
    \myfig{fig/teaser/image_2_retrieval_l00.jpg} &
    {\boxcolor \fbox{ \parbox[c][0.125\textwidth][c]{0.12\textwidth}{\centering \texttt{\textcolor{black}{with jogging path}}}}} \\


    \mycaption{Query Image}&
    \mycaption{$\lambda = 0$} &
    %\mycaption{$\lambda = 0.2$} &
    \mycaption{$\lambda = 0.5$} &
    %\mycaption{$\lambda = 0.8$} &
    \mycaption{$\lambda = 1$} &
    \mycaption{Query Text}\\

\end{tabular}
\vspace{-6pt}
\captionof{figure}{We introduce remote sensing composed image retrieval (RSCIR), a novel and expressive remote sensing image retrieval (RSIR) task integrating both image and text in the search query. We also introduce \ours, a flexible, 
training-free method based on RemoteCLIP~\cite{liu2023remoteclip} utilizing a weighting parameter $\lambda$ for more image- or text-oriented results, with $\lambda \to 0$ or $\lambda \to 1$ respectively. For each \textcolor{imagequerycolor}{query image} and \textcolor{textquerycolor}{query text}, retrieved images shown for $\lambda=0$, $\lambda=0.5$ and $\lambda=1$.}
%offering \textsc{wei}ghted \textsc{com}position 
%~\cite{zhou2018patternnet}
\label{fig:teaser}
%------------------------------------------------------------------------------
\par\vspace{10pt}
%------------------------------------------------------------------------------
}
